IIITT@Dravidian-CodeMix-FIRE2021: Transliterate or translate? Sentiment analysis of code-mixed text in Dravidian languages

Sentiment analysis of social media posts and comments for various marketing and emotional purposes is gaining recognition. With the increasing presence of code-mixed content in various native languages, there is a need for ardent research to produce promising results. This research paper bestows a tiny contribution to this research in the form of sentiment analysis of code-mixed social media comments in the popular Dravidian languages Kannada, Tamil and Malayalam. It describes the work for the shared task conducted by Dravidian-CodeMix at FIRE 2021 by employing pre-trained models like ULMFiT and multilingual BERT fine-tuned on the code-mixed dataset, transliteration (TRAI) of the same, English translations (TRAA) of the TRAI data and the combination of all the three. The results are recorded in this research paper where the best models stood 4th, 5th and 10th ranks in the Tamil, Kannada and Malayalam tasks respectively.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
